Strong Lensing analysis of SPT-CLJ2325$-$4111 and SPT-CLJ0049$-$2440, two Powerful Cosmic Telescopes ($R_E > 40''$) from the SPT Clusters Sample

We report the results from a study of two massive ($M_{500c} > 6.0 \times 10^{14} M_{\odot}$) strong lensing clusters selected from the South Pole Telescope cluster survey for their high Einstein radius ($R_E > 40''$), SPT-CLJ2325$-$4111 and SPT-CLJ0049$-$2440. Ground-based and shallow HST imaging indicated extensive strong lensing evidence in these fields, with giant arcs spanning 18\arcsec\ and 31\arcsec, respectively, motivating further space-based imaging followup. Here, we present multiband HST imaging and ground-based Magellan spectroscopy of the fields, from which we compile detailed strong lensing models. The lens models of SPT-CL\,J2325$-$4111 and SPT-CL\,J0049$-$2440 were optimized using 9, and 8 secure multiple-imaged systems with a final image-plane rms of 0\farcs63 and 0\farcs73, respectively. From the lensing analysis, we measure the projected mass density within 500~kpc of $M(<500 ~{\rm kpc}) = 7.30\pm0.07 \times 10^{14}$$M_{\odot}$, and $M(<500 ~{\rm kpc})=7.12^{+0.16}_{-0.19}\times 10^{14}$ $M_{\odot}$ for these two clusters, and a sub-halos mass ratio of $0.12\pm{0.01}$ and $0.21^{+0.07}_{-0.05}$, respectively. Both clusters produce a large area with high magnification ($\mu\geq 3$) for a source at $z=9$, $A^{lens}_{| \mu | \geq 3 }=4.93^{+0.03}_{-0.04} arcmin^2$, and $A^{lens}_{| \mu | \geq 3 }=3.64^{+0.14}_{-0.10} arcmin^2$ respectively, placing them in the top tier of strong lensing clusters. We conclude that these clusters are spectacular sightlines for further observations that will reduce the systematic uncertainties due to cosmic variance. This paper provides the community with two additional well-calibrated cosmic telescopes, as strong as the Frontier Fields, suitable for studies of the highly magnified background Universe.

==> arcstable_both_original.tex <==
\startlongtable
\begin{deluxetable*}{lllllll} 
\tablecolumns{7} 
\tablecaption{List of lensing constraints \label{tab:arcstable}} 
\tablehead{\colhead{ID} &
            \colhead{R.A.}    & 
            \colhead{Decl.}    & 
            \colhead{$z_{spec}$}     &  
            \colhead{Dist}     &
            \colhead{$\mu$}     & 
%            \colhead{$z_{spec}$}       & 
            \colhead{Notes}       \\[-8pt]
            \colhead{} &
            \colhead{J2000}     & 
            \colhead{J2000}    & 
            \colhead{or $z_{model}$ }       &
            \colhead{(\arcsec)} &
            \colhead{} &
%            \colhead{Reference}       & 
            \colhead{}             }
\startdata 
\multicolumn{3}{l}{\SPTXXIII\ Source 1}& 1.5790 & && GMOS; Single giant arc; SL by nearby galaxy\\
1.1 & 351.296820  & -41.187381 & &0.19&$8.2^{+0.1}_{-0.3}$   & \\ 
1.2 & 351.295943  & -41.187662 & &0.11&$4.4^{+0.4}_{-0.7}$   &  \\ 
11.1 & 351.296463 & -41.187529 & &0.16&$24.5^{+3.1}_{-2.3}$  &  \\ 
11.2 & 351.296232 & -41.187615 & &0.09&$12.7^{+3.0}_{-2.0}$  &  \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 2}& 2.4253 & && FIRE spec of 2.3, from OIII, H$\beta$, H$\alpha$; 2019-12-04\\
20.1 & 351.301880 & -41.192335 & &0.51& $2.5^{+0.2}_{-0.2}$ &  \\ 
20.2 & 351.285884 & -41.202655 & &0.31& $5.0^{+0.1}_{-0.3}$ &  \\ 
20.3 & 351.303568 & -41.209014 & &0.44& $8.4^{+0.3}_{-0.3}$ &  \\ 
20.4 & 351.312449 & -41.197529 & &0.28& $25.1^{+2.7}_{-1.2}$ &  \\ 
20.5 & 351.299833 & -41.202644 & &0.28& $1.4^{+0.2}_{-0.1}$ &  \\ 
21.1 & 351.302765 & -41.192171 & &1.31& $7.7^{+0.7}_{-0.1}$ &  \\ 
21.2 & 351.285764 & -41.202283 & &0.78& $7.6^{+0.7}_{-0.3}$ &  \\ 
21.3 & 351.304206 & -41.208597 & &0.60& $10.2^{+0.5}_{-0.4}$ &  \\ 
21.4 & 351.312034 & -41.197256 & &0.30& $13.1^{+0.3}_{-0.7}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 3}& 3.8180 & && FIRE spec of 3.1, both OIII lines in K-band; 2019-12-05\\
3.1 & 351.306626 & -41.189283 & &0.21&$42.1^{+7.2}_{-2.9}$  &  \\ 
3.2 & 351.301163 & -41.188301 & &0.36& $5.8^{+0.6}_{-0.6}$ &  \\ 
3.3 & 351.285310 & -41.196210 & &0.59& $4.7^{+0.2}_{-0.1}$ &  \\ 
3.4 & 351.301139 & -41.207554 & &0.85& $3.0^{+0.1}_{-0.2}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 4}& 1.3180 & & & FIRE spec of 4.3, H$\alpha$; 2019-12-05 \\
40.1 & 351.291829 & -41.206459 & &1.03& $7.8^{+0.2}_{-0.2}$&\\ 
40.2 & 351.297771 & -41.209536 & &0.56& $3.5^{+0.2}_{-0.3}$ &  \\ 
40.3 & 351.311327 & -41.203079 & &1.19& $8.6^{+0.3}_{-0.2}$ &  \\ 
40.4 & 351.298830 & -41.197679 & &1.03&  $6.7^{+0.2}_{-0.8}$ &  Radial arc\\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 5} &  $1.29\pm{0.01}$ & &&\\
5.1 & 351.293221 & -41.208914 & &0.73& $9.7^{+0.3}_{-0.4}$ & \\ 
5.2 & 351.298529 & -41.210439 & &0.27& $8.9^{+0.4}_{-0.6}$ &  \\ 
5.3 & 351.306435 & -41.208372 & &0.82& $13.0^{+0.4}_{-0.7}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 6} & $7.02\pm{0.20}$ & &&\\
6.1 & 351.313070 & -41.189842 & &1.01& $4.9^{+0.2}_{-0.2}$ & \\ 
6.2 & 351.292582 & -41.189019 & &0.54& $14.4^{+1.1}_{-1.1}$ & \\ 
6.3 & 351.288051 & -41.192324 & &  & $12.0^{+0.4}_{-0.5}$ & \\ 
6.4 & 351.299692 & -41.207262 & &0.91& $2.1^{+0.1}_{-0.1}$ & \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 7}& \nodata & &&\\
7.1$c$ & 351.293554 & -41.194939 & &&  & \\
7.2$c$ & 351.292862 & -41.195442 & &&  & \\
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 8}& $3.00\pm{0.16}$ & &&\\
8.1 & 351.302596 & -41.198158 & &0.42& $7.7^{+0.6}_{-0.7}$ &  Radial arc \\ 
8.2 & 351.301964 & -41.198866 & &0.48& $22.5^{+7.6}_{-4.4}$ &  Radial arc \\ 
8.3 & 351.305018 & -41.194379 & &0.04& $4.0^{+0.4}_{-1.0}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTXXIII\ Source 9}& $1.21\pm{0.01}$ & &&\\
9.1 & 351.305663 & -41.207017 & &0.38& $18.5^{+1.0}_{-0.7}$ & \\ 
9.2 & 351.301553 & -41.208875 & &0.49 & $13.4^{+0.8}_{-0.5}$ & \\ 
9.3 & 351.290113 & -41.205325 & &0.42 & $4.9^{+0.1}_{-0.2}$ & \\ 
\hline 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 1}& 3.0220 & && FIRE spec of 1.2; OIII\\
1.1 & 12.306837 & -24.678576 & 3.0220 &0.32& $6.4^{+0.8}_{-0.4}$ &  \\ 
1.2 & 12.304789 & -24.673793 & &0.31&$6.8^{+1.1}_{-0.8}$  &  \\ 
1.3c& 12.293434 & -24.669124 & && $8.9^{+1.3}_{-0.6}$ & spectroscopy attempted, not confirmed\\
1.4 & 12.290510 & -24.685268 & &0.30& $2.2^{+0.5}_{-0.2}$ &  \\ 
101.1 & 12.306927 & -24.679502 & &0.47& $5.7^{+0.9}_{-0.2}$ &  \\ 
101.3c& 12.293478 & -24.669244 & && $9.8^{+1.5}_{-0.7}$ &  \\
101.4 & 12.290435 & -24.685274 & &0.18& $2.3^{+0.5}_{-0.3}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 2}& $1.52\pm{0.10}$ & &&\\
2.1 & 12.296863 & -24.668930 & &0.15& $19.9^{+4.5}_{-1.3}$ &  \\ 
2.2 & 12.297035 & -24.668981 & &0.14& $4.3^{+1.2}_{-0.7}$ &  \\ 
2.3 & 12.297701 & -24.669017 & &0.22& $5.0^{+0.6}_{-0.4}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 3}& $3.62\pm{0.31}$ & &&\\
3.1 & 12.302022 & -24.681788 & &0.19& $5.5^{+0.7}_{-0.6}$ &  \\ 
3.3 & 12.281064 & -24.672098 & &0.23& $2.5^{+0.2}_{-0.2}$ &  \\ 
3.4 & 12.297052 & -24.680913 & &0.12& $3.7^{+0.6}_{-0.4}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 4}& $3.03\pm{0.16}$ & &&\\
4.1 & 12.284454 & -24.681115 & &0.05& $11.7^{+0.8}_{-0.9}$ &  \\ 
4.3 & 12.303653 & -24.689925 & &0.10& $3.9^{+0.2}_{-0.2}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 5}& $1.37\pm{0.03}$ & &&\\
5.1 & 12.291012 & -24.680759 &  &2.43&$12.8^{+0.9}_{-0.9}$ &  Radial arc\\ 
5.2 & 12.291352 & -24.680671 &  &1.98&$12.9^{+1.0}_{-0.8}$ &  Radial arc\\ 
5.3 & 12.293889 & -24.678894 &  &0.40&$9.1^{+0.8}_{-0.3}$ &  \\ 
5.4 & 12.303297 & -24.684562 &  &1.42&$3.2^{+0.2}_{-0.3}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 6}& 2.368 & && FIRE spec of both 6.1 and 6.2; OIII  \\
6.1 & 12.298507 & -24.681234 & 2.368 &0.11& $71^{+70}_{-7}$ &  Radial arc \\ 
6.2 & 12.298314 & -24.681211 & 2.368 &0.20& $860^{+90}_{-12}$&  Radial arc\\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 7}& $2.30\pm{0.10}$ & &&\\
7.1 & 12.296999 & -24.680492 & &0.02& $4.3^{+0.7}_{-0.4}$ &  \\ 
7.2 & 12.300114 & -24.680802 & &0.62& $4.9^{+1.0}_{-0.4}$ &  \\ 
7.3 & 12.301315 & -24.680923 & &0.54& $3.5^{+0.5}_{-0.3}$ &  \\ 
7.4 & 12.282750 & -24.673044 & &0.01& $2.9^{+0.3}_{-0.1}$ &  \\ 
\hline
\multicolumn{3}{l}{\SPTZERO\ Source 8}& $4.96\pm{0.61}$ & &&\\
8.1 & 12.298777 & -24.688750 & &0.10& $13^{+2}_{-1}$ &  \\ 
8.2 & 12.295079 & -24.689882 & &0.08& $56^{+18}_{-11}$ &  \\ 
\enddata 
\tablecomments{The IDs, positions, and redshifts of lensed galaxies that were used as constraints in this work. Where possible, individual emission knots in each image are identified and used as lensing constraints. 
   %The IDs of images of lensed galaxies are labeled as $AB.X$ where $A$ is a number indicating the source ID (or system name);  $B$ is a number indicating the ID of the emission knot within the system; and $X$ is a number indicating the ID of the lensed image within the multiple image family. 
   {\bf The IDs of images of lensed galaxies are labeled as A.B(.C) where A is the number indicating the source ID (or system name); B is the number indicating the ID of lensed image within the multiple images family; C is a number indicating the ID of emission knot within the image if we used more than one substructure of the images as constraints.}
   $c$ indicates a candidate arc that was not used to constrain the model. {\bf Dist, often called individual rmsi, refers to the distance in the image plane between the image an the projected center of the source. For each system the center of the source is determined by the geometric mean of source plane positions of individual images.}
   }
\end{deluxetable*}

==> spt2325_arcstable_2023.tex <==
\startlongtable
\begin{deluxetable*}{lllll} 
\tablecolumns{5} 
\tablecaption{List of lensing constraints in \SPTXXIII\ \label{tab:arcstable}} 
\tablehead{\colhead{ID} &
            \colhead{R.A.}    & 
            \colhead{Decl.}    & 
            \colhead{$z_{spec}$}     & 
%            \colhead{$z_{spec}$}       & 
            \colhead{Notes}       \\[-8pt]
            \colhead{} &
            \colhead{J2000}     & 
            \colhead{J2000}    & 
            \colhead{}       & 
%            \colhead{Reference}       & 
            \colhead{}             }
\startdata 
\multicolumn{3}{l}{Source 1}& 1.5790 & GMOS; Single giant arc; SL by nearby galaxy\\
1.1 & 351.296820 & -41.187381 & & \\ 
1.2 & 351.295943 & -41.187662 &  &  \\ 
11.1 & 351.296463 & -41.187529 &  &  \\ 
11.2 & 351.296232 & -41.187615 &  &  \\ 
\hline
\multicolumn{3}{l}{Source 2}& 2.4253 & FIRE spec of 2.3, from OIII, Hb, Ha; 2019-12-04\\
20.1 & 351.301880 & -41.192335 &  &  \\ 
20.2 & 351.285884 & -41.202655 &  &  \\ 
20.3 & 351.303568 & -41.209014 &  &  \\ 
20.4 & 351.312449 & -41.197529 &  &  \\ 
20.5 & 351.299833 & -41.202644 &  &  \\ 
21.1 & 351.302765 & -41.192171 &  &  \\ 
21.2 & 351.285764 & -41.202283 &  &  \\ 
21.3 & 351.304206 & -41.208597 &  &  \\ 
21.4 & 351.312034 & -41.197256 &  &  \\ 
\hline
\multicolumn{3}{l}{Source 3}& 3.8180 & FIRE spec of 3.1, both OIII lines in K-band; 2019-12-05\\
3.1 & 351.306626 & -41.189283 &  &  \\ 
3.2 & 351.301163 & -41.188301 &  &  \\ 
3.3 & 351.285310 & -41.196210 &  &  \\ 
3.4 & 351.301139 & -41.207554 &  &  \\ 
\hline
\multicolumn{3}{l}{Source 4}& 1.3180 & FIRE spec of 4.3, Ha; 2019-12-05 \\
40.1 & 351.291829 & -41.206459 & &\\ 
40.2 & 351.297771 & -41.209536 &  &  \\ 
40.3 & 351.311327 & -41.203079 &  &  \\ 
40.4 & 351.298830 & -41.197679 &  &  Radial arc\\ 
\hline
\multicolumn{3}{l}{Source 5} & \nodata &\\
5.1 & 351.293221 & -41.208914 &  & \\ 
5.2 & 351.298529 & -41.210439 &  &  \\ 
5.3 & 351.306435 & -41.208372 &  &  \\ 
\hline
\multicolumn{3}{l}{Source 6} & \nodata &\\
6.1 & 351.313070 & -41.189842 &  & \\ 
6.2 & 351.292582 & -41.189019 &  & \\ 
6.3 & 351.288051 & -41.192324 &  & \\ 
6.4 & 351.299692 & -41.207262 &  & \\ 
\hline
\multicolumn{3}{l}{Source 7}& \nodata &\\
7.1$c$ & 351.293554 & -41.194939 &  & \\
7.2$c$ & 351.292862 & -41.195442 &  & \\
\hline
\multicolumn{3}{l}{Source 8}& \nodata &\\
8.1 & 351.302596 & -41.198158 &  &  Radial arc \\ 
8.2 & 351.301964 & -41.198866 &  &  Radial arc \\ 
8.3 & 351.305018 & -41.194379 &  &  \\ 
\hline
\multicolumn{3}{l}{Source 9}& \nodata &\\
9.1 & 351.305663 & -41.207017 &  & \\ 
9.2 & 351.301553 & -41.208875 &  & \\ 
9.3 & 351.290113 & -41.205325 &  & \\ 
\enddata 
\tablecomments{The IDs, positions, and redshifts of lensed galaxies that were used as constraints in this work. Where possible, individual mission knots in each image are identified and used as lensing constraints. 
   The IDs of images of lensed galaxies are labeled as $AB.X$ where $A$ is a number indicating the source ID (or system name);  $B$ is a number indicating the ID of the emission knot within the system; and $X$ is a number indicating the ID of the lensed image within the multiple image family. $c$ indicates a candidate arc that was not used to constrain the model.}
\end{deluxetable*}
